An Unbiased Transformer Source Code Learning with Semantic Vulnerability Graph

Over the years, open-source software systems have become prey to threat actors. Even as open-source communities act quickly to patch the breach, code vulnerability screening should be an integral part of agile software development from the beginning. Unfortunately, current vulnerability screening techniques are ineffective at identifying novel vulnerabilities or providing developers with code vulnerability and classification. Furthermore, the datasets used for vulnerability learning often exhibit distribution shifts from the real-world testing distribution due to novel attack strategies deployed by adversaries and as a result, the machine learning model's performance may be hindered or biased. To address these issues, we propose a joint interpolated multitasked unbiased vulnerability classifier comprising a transformer "RoBERTa" and graph convolution neural network (GCN). We present a training process utilizing a semantic vulnerability graph (SVG) representation from source code, created by integrating edges from a sequential flow, control flow, and data flow, as well as a novel flow dubbed Poacher Flow (PF). Poacher flow edges reduce the gap between dynamic and static program analysis and handle complex long-range dependencies. Moreover, our approach reduces biases of classifiers regarding unbalanced datasets by integrating Focal Loss objective function along with SVG. Remarkably, experimental results show that our classifier outperforms state-of-the-art results on vulnerability detection with fewer false negatives and false positives. After testing our model across multiple datasets, it shows an improvement of at least 2.41% and 18.75% in the best-case scenario. Evaluations using N-day program samples demonstrate that our proposed approach achieves a 93% accuracy and was able to detect 4, zero-day vulnerabilities from popular GitHub repositories.

==> sections/algorithms_pg5.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ALGORITHM I
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\begin{algorithm}[b]
\caption{Create API\_ASSIGNMENT}\label{alg:oe}
\begin{algorithmic}[1]

\Require \textit{code, adj\_matrix}: List of Tokens from Code
\Ensure SVG
\Procedure{\textit{API\_ASSIGNMENT}}{$tokens$}%\Comment{The g.c.d. of a and b}
%\State $params \gets getCmdLineParams(tokens)$
\State $tokens \gets Tokenizer(code)$
\For{$token$ in $tokens$}
    %\State $type \gets getTokenType(token)$
    \If{$token$ in $assignment_operators$}
        \State $left \gets getPrevToken(token)$
        \State $right \gets getNextTokens(token)$
        
        \State $adj_matrix[left][right] \gets 1$
        
    \EndIf
\EndFor
\State \Return $adj\_matrix$
\EndProcedure
\end{algorithmic}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ALGORITHM II
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\begin{algorithm}[t]
\caption{Create CHECK\_VALUE}\label{alg:cv}
\begin{algorithmic}[1]

\Require \textit{code, adj\_matrix}: List of Tokens from Code
\Ensure SVG
\Procedure{\textit{CHECK\_VALUE}}{$tokens$}
\State $tokens \gets Tokenizer(code)$
\State $params \gets getCmdLineParams(tokens)$
\For{$token$ in $tokens$}
    \State $type \gets getTokenType(token)$
    \If{$type$ in $condition$}
        \State $next\_token \gets getNextToken(token)$
        \State $next\_block\_tokens \gets getNextBlockToken(token)$
        \If{$next\_token$ is subset $params$ and \\
        $next\_block\_tokens$ is subset $params$
        }
            \State $adj_matrix[condition][next\_token] \gets 1$
            \State $adj_matrix[condition][next\_block\_tokens] \gets 1$
        \EndIf
    \EndIf
    
\EndFor
\State \Return $adj\_matrix$
\EndProcedure
\end{algorithmic}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/algorithms_pg6.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ALGORITHM III
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\begin{algorithm}[!ht]
\caption{OUT\_OF\_SCOPE and RACE\_CONDITION}\label{alg:sr}
\begin{algorithmic}[1]
\Require \textit{tokens, adj\_matrix}: List of Tokens from Code
\Ensure Semantic Graph
\Procedure{\textit{SCOPE\_RACE}}{$tokens$}
\State $scope:Dictionary$
%\State $node \gets root$
\For{$token$ in $tokens$}%\Comment{We have the answer if r is 0}
    \If{$scope[token]$ is $done$}
        \State  $adj\_matrix["free"][token] \gets 1$
    \EndIf
    \State $stack.push(token)$
    \If{$token pair match$}
        \State $pair\_token \gets stack.pop()$
    \EndIf
        \If{$token$ is $"free"$}
        \State $next\_token \gets getNextToken(token)$
        \State $scope[next\_token] \gets end$
    \EndIf
\EndFor\label{euclidendwhile1}
\State \Return $adj\_matrix$
\EndProcedure
\end{algorithmic}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Algorithm IV
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[t]
\caption{Create CMD\_INJECTION}\label{alg:ci}
\begin{algorithmic}[1]

\Require \textit{code, adj\_matrix}: List of Tokens from Code



\Ensure SVG



\Procedure{\textit{CMD\_INJECTION}}{$tokens$}%\Comment{The g.c.d. of a and b}
\State $tokens \gets Tokenizer(code)$
\State $params \gets getCmdLineParams(tokens)$

\For{$token$ in $tokens$}
    \State $type \gets getTokenType(token)$
    \If{$type$ in $condition$}
        \State $next\_token \gets getNextToken(token)$
        \If{$next\_token$ is subset $params$}
            \State $adj_matrix[condition][next\_token] \gets 1$
        \EndIf
    \EndIf
    
\EndFor

\State \Return $adj\_matrix$
\EndProcedure




\end{algorithmic}
\end{algorithm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Algorithm V
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\begin{algorithm}[!ht]
\caption{SVG Creation Algorithm}\label{alg:graph}
\begin{algorithmic}[1]

\Require \textit{code, edge\_length}: 

\Ensure Adjacency Matrix

\Procedure{\textit{SVG\_Generation}}{$code$}%\Comment{The g.c.d. of a and b}

\State $tokens \gets RoBERTaTokenizer(code)$
\State $adj\_matrix \gets [ ][ ]$
\State $var\_list \gets []$
\State $cond\_statement$ = $for/if/while/else/else if$
%\State $CWE\_EDGE\_LIST \gets [Egde Types from Table \ref{tab:graph}]$
%\State $node \gets root$

\While{$token$ in $tokens$}%\Comment{We have the answer if r is 0}
    \State $type = checkTokernType(token)$
    \If{$type$ is $"variable"$}
        \State $var\_list.append(token)$
        \If{$token$ exists in $var\_list$}
            \State $prev\_token  \gets getPrevTok(token)$
            \State $adj\_matr[token][prev\_token]  \gets 1$
        \EndIf
        
    \EndIf
    
    \If{$token$ in $assignment_operators$}
        \State $left \gets getPrevToken(token)$
        \State $right \gets getNextToken(token)$
        
        \State $adj_matrix[left][right] \gets 1$
        
    \EndIf
    
    \Comment{Control Flow Edge Generate}
    \State $next \gets getNextToken(token)$
    \State $adj\_matr[token][next\_token]  \gets 1$
    \If{$type$ is in $"cond\_statements"$}
        
        \State $next\_token  \gets getNextBlockToken(token)$
        
        \State $adj\_matr[token][next\_token]  \gets 1$
           
            
        
        
    \EndIf 
\EndWhile\label{euclidendwhile1}

\State $OPERATION\_EDGE(tokens)$
\State $CHECK\_VALUE(tokens)$
\State $SCOPE\_RACE(tokens)$
\State $CMD\_INJECTION(tokens)$
\State $SEQUENTIAL\_TOKEN\_EDGE(tokens)$
 




\EndProcedure
\end{algorithmic}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sections/backup.tex <==
% ################  This section is merged with Proposed Model section  ######################### %

Our objective is to find vulnerabilities in source code at the function level in a real-world environment. However, considering source code only as a sequence of tokens, similar to Natural Language Processing (NLP), is not very helpful for detecting vulnerabilities, as programming languages are more structured than natural languages, and program output may produce different behaviors for different input and memory states, which are not present in natural languages. Figure \ref{fig:code} exemplifies this situation that consecutive lines may not contribute to vulnerability. In order to identify vulnerability precisely, we need to understand the relation between tokens of distant statements. The effect of a distant statement may cause a vulnerability. Alternatively, it can be caused due to incorrect input from the user during program execution. Hence we will formalize the problem as a binary classification problem using graph-based analysis to detect long-term token dependencies by leveraging graph edges. 
\hfill \break

\textbf{Problem Definition:\color{red} Embedding X comes from RoBERTa \color{black}} Some vulnerability detectors detect vulnerability at a file-level granularity\cite{dam2018automatic}, and other enterprise-based tools like \textit{CheckMarx} and \textit{Coverity} depend on a fully compilable code to run vulnerability analysis. As a result, these analyses are mostly language-dependent and cannot be generalized to another programming language. Hence we decided to use function level granularity for vulnerability detection, which will also help us extend our work for different programming languages in the future. However, these functions can not be compiled standalone without the help of other header files in the compilation directory. Since, in our study, we employed a unique token-focused graph generation with data and control flow, we can exploit the advantage of having a graph structure of source code with rich feature representation from data and control flow to detect the vulnerability of code from a project still under development.

In order to define the problem formally, let a code snippet be defined as $\{(s_i, v_i)| s_i \in S, v_i \in V \}$ and $i \in \{1, 2, 3, ..., n \}$, where
$ S $ denotes the set of functions/methods which may or may not be compilable as standalone program, $V = \{ 0, 1 \}$ as the set of labels corresponding to each function. When the value is 1 it means the code is vulnerable and 0 otherwise. $n$ is the total number of function/code snippets. Considering $s_i$ as a function, 

we convert this function into a heterogeneous multi-edged graph $G_i (N, X, A) \in \mathbb{G}$, where $N$ is the set of $v$ nodes in a graph,  $X \in \mathbb{G}\textsuperscript{\textit{v x d}} $ defined as $d$ dimensional feature vector of each node $v$ in the graph and $A$ is the adjacency matrix where, $A \in \{ 0, 1 \} $. Here, 1 means there is an edge between node $v_i$ and $v_{i+1}$ and 0 otherwise. 

For this problem we are defining three types of edges, token-based edges, data flow and control flow edges. We put all the edge information in our adjacency matrix. Our goal is to learn mapping from graph $\mathbb{G}$ to vulnerability $V$ such that, $ \mathfrak{f} : \mathbb{G} \Rightarrow V $. Vulnerability prediction function $\mathfrak{f}$ can be formally defined as:

\color{blue}
%%  Comment from Dr Rad.
We need an encoding $e(s_i) cap$ technique that we $s_i$ generate embedidng of code snippet. $P e(s_i)$ and compare with $v_i$ labeled. P is the vulenrability classifier with regularization.
Change the formula accordingly
Embedding $e_{roberta} to generate initial X$
In Fig 3, call embedding of RoBERTa
Check autoencoder.
Figure 2, small code snippet

Remove Bias
%%
\color{black}

\[ min \sum_{i=1}^{n} \mathcal{L} (\mathfrak{f}(G_i (N, X, E), v_i | f_i)) + \mathfrak{w_i}\lambda  \] 
where $\mathcal{L(.)}$ is the loss function we used for our experiments, $\mathfrak{w_i}$ is regularization and $\lambda$ is adjustable weight which is learned during training.





%\begin{figure}[ht!]
%\begin{minipage}[b]{1.0\linewidth}
%  \centering
%  \centerline{\includegraphics[width=8cm, height=10cm]{images/ast.png}}
  %\vspace{2.0cm}
%  \caption{A sample AST}
%  \label{fig:ast}
%\end{minipage}
%\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{subfigure}[b]{0.45\textwidth}
            \centering
            \lstinputlisting[language=c++]{code_samples/vul.c}

            %\vspace{2.0cm}
            \caption{Sample code from NVD/SARD Dataset Showing a Buffer Overflow Vulnerability}
            \label{fig:vul}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.45\textwidth}
            \centering
            \lstinputlisting[language=c++]{code_samples/ben.c}

            %\vspace{2.0cm}
            \caption{Sample code from NVD/SARD Dataset Fixing the Buffer Overflow Vulnerability}
            \label{fig:ben}
        \end{subfigure}
        
        



\begin{itemize}
    \item We propose RoBERTA-GCN, a deep learning-based model for vulnerability detection with a weighted loss function that takes advantage of both pre-trained representation and  GCN for transductive learning. We leverage RoBERTa to generate the token representation. The GCN layers generate the final embeddings for vulnerability classification.  
    
    \item We propose a focal loss function by assigning smaller weights to the loss for majority class cases and larger weights for minority class examples due to the imbalanced nature of the real-world vulnerability dataset. We demonstrated empirically that our model with focal loss outperforms conventional loss functions, making the model less biased toward majority class.
    
    \item We investigated the effectiveness of our model on three unique datasets by training on one dataset and testing on another to demonstrate the robustness of each dataset. Furthermore, utilizing the most recent real-world vulnerabilities from the National Vulnerability Database (NVD), we evaluated our model on a more recent dataset and demonstrated our model's capacity to generalize vulnerabilities by detecting the semantic meaning of code.
    
    
    %\item Since our graph representation contains rich code representations, we leverage this graph for vulnerability classification. We also did an empirical study on the effect of AST-based graph construction compared to our flat token-based graph construction on vulnerability detection tasks.
\end{itemize}


\begin{comment}

\begin{itemize}
    \item \textbf{CWE-787 Out-of-bounds Write:} The software writes data past the specified buffer's end or before its commencement. This unspecified writing on buffer typically results in data corruption, a system crash, or code execution.
    
    \item \textbf{CWE-20 Improper Input Validation:} The program accepts input or data but fails to validate it. As a result, altered control flow, arbitrary control of a resource, or execution of arbitrary code may occur. 
    
    \item \textbf{CWE-125 Out-of-bounds Read:} The program reads data before or after the scope of the buffer, resulting in out-of-bounds memory, causing excessive data to be read, and generating a segmentation fault or buffer overflow.
    
    \item \textbf{CWE-78 Improper Neutralization of Special Elements used in an OS Command:} The software produces all or a portion of an OS command using externally-influenced information from an upstream component but fails to neutralize or neutralize incorrectly, allowing attackers to execute unexpected commands directly.
    
    \item \textbf{CWE-416 Use After Free:} Referring to freed memory might cause a program to crash, use unexpected variables, or execute code.
    
    \item \textbf{CWE-476 NULL Pointer Dereference:} A NULL pointer dereference occurs when an application dereferences a pointer that it assumes to be valid but is instead NULL, resulting in a usual crash or exit.
    
    \item \textbf{CWE-190 Integer Overflow or Wraparound:} The software conducts a calculation that may result in an integer overflow or wraparound if the logic expects that the result will always be greater than the initial number.
    
    \item \textbf{CWE-798 Use of Hard-coded Credentials:} The software has hard-coded credentials for its inbound authentication, giving the attackers an easy way to gain the credentials.
    
    \item \textbf{CWE-77 Improper Neutralization of Special Elements used in a Command:} The software produces all or part of a command using externally influenced information from an upstream component but fails to neutralize or neutralize certain aspects that could change the intended command when sent to a downstream component.
    
    \item \textbf{CWE-119 Improper Restriction of Operations within the Bounds of a Memory Buffer:} The software operates on a memory buffer but can read from or write to memory locations beyond the intended buffer boundary. As a result, an attacker may be able to run arbitrary code, disrupt the intended control flow, read sensitive data, or cause the system to crash.
    
    \item \textbf{CWE-362 Concurrent Execution using Shared Resource with Improper Synchronization:}  The program contains a code sequence that can run concurrently with other codes. However, the code sequence requires temporary, exclusive access to a shared resource with security implications, such as recording whether a user is authenticated or modifying crucial state information that an outsider should not modify. 
    
    \item \textbf{CWE-400 Uncontrolled Resource Consumption:} The application does not adequately control the allocation and maintenance of a restricted resource, allowing an attacker to manipulate the number of resources consumed, ultimately leading to the depletion of available resources. 
    
    
    
    
\end{itemize}

\end{comment}




\begin{table}[ht]
\centering
\caption{Ablation Studies on the components of RoBERTa-GCN}
\label{tab:ablation}
\begin{tabular}{ll}
\toprule
\multicolumn{1}{l}{\textbf{Methods}} & \textbf{Accuracy} \\
\midrule
RoBERTa-GCN   & -   \\
w/o AST   & -   \\
w/o Focal Loss   & -   \\
\bottomrule
\end{tabular}
\end{table}




CWE-787: Out-of-bounds Write & 10 & 10 & The software writes data past the specified buffer's end or before its causing data corruption\\

CWE-20: Improper Input Validation  & 2 & 2 & The program accepts input or data but fails to validate resulting in altered control flow. \\

CWE-125: Out-of-bounds Read & 1 & 1 & The program reads data before or after the scope of the buffer, resulting in out-of-bounds memory \\

CWE-78: Improper Neutralization of Special Elements used in an OS Command  & 14 & 14 & The software produces a portion of an OS command using externally-influenced information to execute unexpected commands.\\

CWE-416: Use After Free	 & 4 & 4 & Referring to freed memory causing a program to crash, use unexpected variables, or execute code.\\

CWE-476: NULL Pointer Dereference & 3 & \textbf{2}  &   Occurs when an application dereferences a pointer that it assumes to be valid resulting in a usual crash \\

CWE-190: Integer Overflow or Wraparound & 9 & 9 & Software conducts a calculation that may result in an integer overflow or wraparound \\

CWE-798:Use of Hard-coded Credentials & 2 & 2 & Hard-coded credentials used for its inbound authentication, providing the attackers gain the credentials. \\

CWE-77:Improper Neutralization of Special Elements used in a Command  & 2 & 2 & Externally influenced information or command are executed, causing system disruption.\\

%CWE-119 & - & - & The software executes operations on a memory buffer but can read from or write to memory locations outside the buffer's intended border.\\

CWE-362: Concurrent Execution using Shared Resource with Improper Synchronization & 2 & 2 & Code sequence that can be executed concurrently with other code causing race condition to appear.\\

CWE-400: Uncontrolled Resource Consumption & 5 & 5 & Software weakly manages restricted resources, allowing an attacker to influence resources.\\




%% Following is a test eqn
\begin{equation}
\label{eqn:testlabel}
R(w_i) = \lambda \frac{1}{2} || w_i ||^2
\end{equation}


\begin{table}[hbt!]
\centering
\caption{Vulnerability Detection Using Focal Loss. This table shows the effectiveness of our model using the focal loss function. Since only ReVEAL is imbalanced, we only use this dataset for our results.}
\label{fig:focal}
\begin{tabular} {p{0.08\textwidth}
                 p{0.10\textwidth}
                 p{0.04\textwidth}
                 p{0.04\textwidth}
                 p{0.04\textwidth}
                 p{0.04\textwidth}}
\toprule
\textbf{Model}                      & \textbf{Input}                          & \textbf{Acc.}          & \textbf{Prec.}         & \textbf{Recall}        & \textbf{F1}    \\ \midrule
Russell et al.             & Token                          & 90.98         & 24.63         & 10.91         & 15.24 \\
VulDeePecker               & \multirow{2}{*}{Slice + Token} & 89.05         & 17.68         & 13.87         & 15.7  \\
SySeVR                     &                                & 84.22         & 24.46         & 40.11         & 30.25 \\
Devign                     & CPG                            & 88.41         & 34.61         & 26.67         & 29.87 \\
\textbf{RoBERTa-GCN w/ WL} & Semantic Vulnerability Graph                 & 88.07         &46.34          & 49.14         & 47.31 \\
\textbf{RoBERTa-GCN w/ FL} & Semantic Vulnerability Graph       & \textbf{89.88} & \textbf{57.52} & \textbf{50.20} & \textbf{47.91}     \\ \bottomrule


\end{tabular}
\end{table}



% New Table

%\paragraph{\textbf{AST Generation:}} In Figure \ref{fig:ast} we show an example of C++ code with its equivalent AST. Rounded-edged rectangles are leaf nodes, and sharp-edged are intermediate tokens. We used \color{red} \textit{Tree Sitter} \color{black} library to generate the AST. Also, AST provides richer syntax information. For example, if we consider the sub-tree "\textit{assignment} $ \Rightarrow $ \textit{i\_n} ", we can immediately understand that the variable \textit{i\_n} is assigned some value, and if traverse the tree more, we can figure out what value is assigned along with its data types. These pieces of information are likely to be used as additional information, enhancing the model's representation. However, a large program using AST edges as an input for the GCN becomes computationally very expensive. In order to address this problem, we flatten the AST using pre-order traversal to create a unique token-based graph construction. Algotithm \ref{alg:euclid} shows the procedure we used to flatten the AST.

%\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%\renewcommand{\algorithmicensure}{\textbf{Output:}}
%\begin{algorithm}
%\caption{AST Flattening Algorithm}\label{alg:euclid}
%\begin{algorithmic}[1]

%\Require \textit{root}: The root node of AST
%\Ensure Flattened Version of AST

%\Procedure{\textit{F}}{$root$}%\Comment{The g.c.d. of a and b}

%\State $flattened\_list \gets []$
%\State $node \gets root$

%\If{$root$ is $leaf\_node$}
%    \State $flattened\_list.append \gets name$
%\Else
%    \State $flattened\_list.append \gets name.left$
%    \While{$child$ in children of $root$}%\Comment{We have the answer if r is 0}
%        \State $F(child)$
        
%\EndWhile\label{euclidendwhile}
%    \State $flattened\_list.append \gets name.right$
    
%\EndIf 
%\EndProcedure
%\end{algorithmic}
%\end{algorithm}




%%%%%%%%%%%%% Final Algorithm   %%%%%%%%%%%%%%%%%%%%%%%%%%



\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\begin{algorithm}
\caption{CWE Graph Helper Methods}\label{alg:graph2}
\begin{algorithmic}[1]

\Require \textit{tokens, adj\_matrix}: List of Tokens from Code



\Ensure Semantic Graph

\Procedure{\textit{SCOPE\_RACE}}{$tokens$}%\Comment{The g.c.d. of a and b}


\State $scope:Dictionary$
%\State $node \gets root$

\While{$token$ in $tokens$}%\Comment{We have the answer if r is 0}
    \If{$scope[token]$ is $done$}
        \State  $adj\_matrix["free"][token] \gets 1$
    \EndIf
    \State $stack.push(token)$
    \If{$token pair match$}
        \State $pair\_token \gets stack.pop()$
        
        
    \EndIf
        \If{$token$ is $"free"$}
        \State $next\_token \gets getNextToken(token)$
        \State $scope[next\_token] \gets end$
    \EndIf
    
\EndWhile\label{euclidendwhile1}

\State \Return $adj\_matrix$
 
\EndProcedure

\Procedure{\textit{CHECK\_VALUE}}{$tokens$}%\Comment{The g.c.d. of a and b}

% write here

\State $params \gets getCmdLineParams(tokens)$
 
\For{$token$ in $tokens$}
    \State $type \gets getTokenType(token)$
    \If{$type$ in $condition$}
        \State $next\_token \gets getNextToken(token)$
        \State $next\_block\_tokens \gets getNextBlockToken(token)$
        \If{$next\_token$ is subset $params$ and \\
        $next\_block\_tokens$ is subset $params$
        }
            \State $adj_matrix[condition][next\_token] \gets 1$
            \State $adj_matrix[condition][next\_block\_tokens] \gets 1$
        \EndIf
    \EndIf
    
\EndFor

\EndProcedure


\Procedure{\textit{CMD\_INJECTION}}{$tokens$}%\Comment{The g.c.d. of a and b}

\State $params \gets getCmdLineParams(tokens)$

\For{$token$ in $tokens$}
    \State $type \gets getTokenType(token)$
    \If{$type$ in $condition$}
        \State $next\_token \gets getNextToken(token)$
        \If{$next\_token$ is subset $params$}
            \State $adj_matrix[condition][next\_token] \gets 1$
        \EndIf
    \EndIf
    
\EndFor


\EndProcedure


\Procedure{\textit{OPERATION\_EDGE}}{$tokens$}%\Comment{The g.c.d. of a and b}

%\State $params \gets getCmdLineParams(tokens)$

\For{$token$ in $tokens$}
    %\State $type \gets getTokenType(token)$
    \If{$token$ in $operators$}
        \State $left \gets getPrevToken(token)$
        \State $right \gets getNextTokens(token)$
        
        \State $adj_matrix[left][right] \gets 1$
        
    \EndIf
    
\EndFor


\EndProcedure


\Procedure{\textit{SEQUENTIAL\_TOKEN\_EDGE}}{$tokens$}%\Comment{The g.c.d. of a and b}

%\State $params \gets getCmdLineParams(tokens)$



\For{$token$ in $tokens$}
    \State $nearbyTokens \gets getNearbyTokens(length)$
    \For{$next\_token$ in $nearbyTokens$}
        \If{$adj\_matr[token][next\_token]$ = $0$}
            \State $adj\_matr[token][next\_token] = 1$
        \EndIf
    \EndFor
    
    %\Comment{Logic For CWE Edges}
\EndFor


\EndProcedure

\end{algorithmic}
\end{algorithm}




\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

\lstdefinestyle{mystyle}{
    %backgroundcolor=\color{backcolour},   
    %commentstyle=\color{codegreen},
    %keywordstyle=\color{magenta},
    %numberstyle=\tiny\color{codegray},
    %stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2
}

\lstset{style=mystyle}



\begin{figure*}
        \centering
        \begin{subfigure}[b]{0.475\textwidth}
            \centering
            \includegraphics[width=\textwidth]{eurosp2023-template/images/DF.pdf}
            \caption[]%
            {{\small Data Flow Edges Only}}    
            \label{fig:df}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.475\textwidth}  
            \centering 
            \includegraphics[width=\textwidth]{eurosp2023-template/images/CF.pdf}
            \caption[]%
            {{\small Control Flow Edges Only}}    
            \label{fig:cf}
        \end{subfigure}
        \vskip\baselineskip
        \begin{subfigure}[b]{0.475\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{eurosp2023-template/images/CWE.pdf}
            \caption[]%
            {{\small CWE Edges Only}}    
            \label{fig:cw}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.475\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{eurosp2023-template/images/combined.pdf}
            \caption[]%
            {{\small Combined Edges}}    
            \label{fig:all}
        \end{subfigure}
        \caption[ The average and standard deviation of critical parameters ]
        {\small We show Data Flow, Control Flow and CWE individually in Figure \ref{fig:df}, \ref{fig:df} and \ref{fig:cw}. Figure \ref{fig:all} shows, how the graph would look like, when they are combined. However for reasons of simplicity, we ignored the SEQUENTIAL\_TOKEN\_EDGE} 
        \label{fig:explain}
\end{figure*}



%%%%%%%%%%%%%%%%%%%%%%%%Test Going Up%%%%%%%%%%%%%%%%%%%%

\begin{table*}[ht]
\centering
\caption{Definition of Rule-based Edge Tags  Generated from CWE Vulnerability Knowledge Repository}
%\label{tab:graph}
\begin{tabular}{p{0.20\textwidth}
                p{0.17\textwidth}
                p{0.45\textwidth}
                 }
\toprule
\multicolumn{1}{l}{\textbf{CWE Number}} & \textbf{CWE Edge Type} & \textbf{Short Description} \\
\midrule

%DATA\_FLOW  &   CWE-787,    &   Desc.   \\
% ASSIGNEMNT_EDGE
% OUT_OF_SCOPE
% NEXT_TOKEN
% CHECK_VALUE
% HARD_CODED_ASSIGNMENT/FORCED_ASSIGNMENT


125, 119, 704, 369, 798, 287, 170, 676 & OPERATION\_EDGE     & Captures mathematical operations during assignment. \\

20, 190, 400, 665, 476  & CHECK\_VALUE     & Check value before assignment operations \\

416, 125, 404, 666 & OUT\_OF\_SCOPE     & Usage of variable after free'd. \\

77, 78, 74, 88, 506 & CMD\_INJECTION     & Check before executing a command line argument \\

362, 662, 573, 400 & RACE\_CONDITION     & An exclusive variable used out of synchronization  \\


\bottomrule
\end{tabular}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{table}[t]
\centering
\caption{Models Performance when Tested on Different Dataset. This table shows the performance of our model when we train the model on one dataset and test it on a different dataset.}
\label{tab:zero-shot}
\begin{tabular}{p{0.09\textwidth}
                 p{0.10\textwidth}
                 %p{0.09\textwidth}
                 p{0.03\textwidth}
                 p{0.03\textwidth}
                 p{0.03\textwidth}
                 p{.03\textwidth}}
\toprule
\textbf{Training Data}                       & \textbf{Evaluate Data}     & \textbf{Acc.}     & \textbf{Prec.}      & \textbf{Recall}     & \textbf{F1}        \\ \midrule

\multirow{2}{*}{ReVEAL}             & D2A               & 47.55    & 48.97     & 49.27       & 44.41     \\
                                    & FFMpeg+Qemu       & 55.01    & 53.65     & 52.45       & 49.39     \\ \midrule
                                                    
\multirow{2}{*}{D2A}                & FFMpeg+Qemu       & 53.40    & 52.67     & 52.45       & 51.86     \\
                                    & ReVEAL            & 68.97    & 48.58     & 47.05       & 46.22     \\ \midrule                                                    
                                                    
\multirow{2}{*}{FFMpeg+Qemu}        & ReVEAL            & 73.75    & 52.66     & 55.18       & 51.93     \\
                                    & D2A               & 53.64    & 52.80     & 52.33       & 50.83     \\ \bottomrule



\end{tabular}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\begin{algorithm}[!ht]
\caption{Graph Creation Algorithm}\label{alg:graph}
\begin{algorithmic}[1]

\Require \textit{code, edge\_length}: 

\Ensure Adjacency Matrix

\Procedure{\textit{SVG\_Generation}}{$code$}%\Comment{The g.c.d. of a and b}

\State $tokens \gets RoBERTaTokenizer(code)$
\State $adj\_matrix \gets [ ][ ]$
\State $var\_list \gets []$
\State $cond\_statement$ = $for/if/while/else/else if$
%\State $CWE\_EDGE\_LIST \gets [Egde Types from Table \ref{tab:graph}]$
%\State $node \gets root$

\While{$token$ in $tokens$}%\Comment{We have the answer if r is 0}
    \State $type = checkTokernType(token)$
    \If{$type$ is $"variable"$}
        \State $var\_list.append(token)$
        \If{$token$ exists in $var\_list$}
            \State $prev\_token  \gets getPrevTok(token)$
            \State $adj\_matr[token][prev\_token]  \gets 1$
        \EndIf
        
    \EndIf
    
    \If{$token$ in $assignment_operators$}
        \State $left \gets getPrevToken(token)$
        \State $right \gets getNextToken(token)$
        
        \State $adj_matrix[left][right] \gets 1$
        
    \EndIf
    
    \Comment{Control Flow Edge Generate}
    \State $next \gets getNextToken(token)$
    \State $adj\_matr[token][next\_token]  \gets 1$
    \If{$type$ is in $"cond\_statements"$}
        
        \State $next\_token  \gets getNextBlockToken(token)$
        
        \State $adj\_matr[token][next\_token]  \gets 1$
           
            
        
        
    \EndIf 
\EndWhile\label{euclidendwhile1}

\State $OPERATION\_EDGE(tokens)$
\State $CHECK\_VALUE(tokens)$
\State $SCOPE\_RACE(tokens)$
\State $CMD\_INJECTION(tokens)$
\State $SEQUENTIAL\_TOKEN\_EDGE(tokens)$
 




\EndProcedure
\end{algorithmic}
\end{algorithm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\caption{Definition of Rule-based Edge Tags  Generated from CWE Vulnerability Knowledge Repository}
\begin{tabular}{p{0.06\textwidth}
                p{0.04\textwidth}
                p{0.13\textwidth}
                p{0.15\textwidth}
                 }

\toprule

\textbf{CWE Number}     & \textbf{Total Count} & \textbf{CWE Edge Category}                    & \textbf{Short Description}                                                                                                   \\ \midrule
Non-Vulnerable & 138522      & \multirow{6}{*}{OPERATION\_CONSTRAINT} & \multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}Captures mathematical \\ operations during \\ assignments.\end{tabular}} \\
119            & 18618       &                                  &                                                                                                                     \\
704            & 5251        &                                  &                                                                                                                     \\
369            & 289         &                                  &                                                                                                                     \\
170            & 45          &                                  &                                                                                                                     \\ 
676            & 61          &                                  &                                                                                                                     \\ \midrule
20             & 2703        & \multirow{5}{*}{CHECK\_VALUE}    & \multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}Check value before \\ assignment operations\end{tabular}}                \\
190            & 326         &                                  &                                                                                                                     \\
400            & 3324        &                                  &                                                                                                                     \\
665            & 2022        &                                  &                                                                                                                     \\
476            & 1701        &                                  &                                                                                                                     \\  \midrule
404            & 2058        & \multirow{2}{*}{OUT\_OF\_SCOPE}  & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Usage of variable \\after free’d.\end{tabular}}                      \\
666            & 580         &                                  &                                                                                                                     \\ \midrule
74             & 4021        & \multirow{2}{*}{CMD\_INJECTION}  & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Check before executing \\a command line argument\end{tabular}}         \\
506            & 421         &                                  &                                                                                                                     \\ \midrule
362            & 211         & \multirow{3}{*}{RACE\_CONDITION} & \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}An exclusive \\ variable used out \\ of synchronization\end{tabular}}    \\
662            & 221         &                                  &                                                                                                                     \\
573            & 331         &                                  &                                                                                                                     \\ \midrule
\label{tab:graph}
\end{tabular}
\end{table}




\begin{figure*}[ht]
    %\begin{framed}
        %\centering
        %test
        \begin{subfigure}[t]{0.47\textwidth}
            %\centering
            %\lstinputlisting[language=c++]{code_samples/ben.c}
            \includegraphics[width=\textwidth]{eurosp2023-template/images/vuln.pdf}
            %\vspace{2.0cm}
            \caption{Vulnerable Code with Output from Classifier}
            \label{fig:g_vul}
        \end{subfigure}
        \hfill
        \begin{subfigure}[t]{0.47\textwidth}
            %\centering
            %\lstinputlisting[language=c++]{code_samples/ben.c}
            \includegraphics[width=\textwidth]{eurosp2023-template/images/fix.pdf}
            %\vspace{2.0cm}
            \caption{Non-Vulnerable Code with Output from Classifier}
            \label{fig:g_ben}
        \end{subfigure}
    %\end{framed}
    \caption{Figure \ref{fig:g_vul} depicts vulnerable code  with its SVG and Figure \ref{fig:g_ben} depicts the patched/fixed code with its SVG. The vulnerability exists when the code attempts to execute \textit{strcpy} by copying t he variable \textit{hp} without checking the assignee variable size, as indicated by the green edges in figure \ref{fig:g_vul}. When we examine the graph from figure \ref{fig:g_ben}, we can see that the red edge neutralizes the vulnerability by verifying the variable's size prior to assignment.}
    \label{fig:code}
\end{figure*}




% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[]
\caption{A metadata of our curated VulF dataset with their corresponding CWE number, LSTD Edge Category and Description}
\begin{tabular}{p{0.08\textwidth}
                p{0.04\textwidth}
                p{0.18\textwidth}
                p{0.60\textwidth}
                 }

\toprule

\textbf{CWE Label}     & \textbf{Number of Functions} & \textbf{LSTD Edge Category} & \textbf{Description}                                                                                                                   \\ \midrule
Non-Vulnerable & 138522      & None & None                                                                                                                          \\ \midrule

119            & 18618      & \multirow{5}{*}{OPERATION\_CONSTRAINT} & The software performs operations on a memory buffer, but it can read from or write to a memory location that is outside of the intended boundary of the buffer.
 \\
                                                                     
704            & 5251        &  & The software does not correctly convert an object, resource, or structure from one type to a different type.
                                                                                                                                                    \\
369            & 289         &   & The product divides a value by zero.
                                                                                                                                                    \\
170            & 45          &                                                                                                                                                       \\ 
676            & 61          &                                                                                                                                                       \\ \midrule
20             & 2703        & \multirow{5}{*}{CHECK\_VALUE}     \\
190            & 326         &                                                                                                                                                       \\
400            & 3324        &                                                                                                                                                      \\
665            & 2022        &                                                                                                                                                   \\
476            & 1701        &                                                                                                                                                   \\  \midrule
74             & 4021        & \multirow{2}{*}{CMD\_INJECTION}  \\
506            & 421         &                                                                                                                                                     \\ \midrule
404            & 2058        & \multirow{2}{*}{OUT\_OF\_SCOPE}  \\
666            & 580         &                                                                                                                                                      \\ \midrule

362            & 211         & \multirow{3}{*}{RACE\_CONDITION}  \\
662            & 221         &                                                                                                                                                      \\
573            & 331         &                                                                                                                                                       \\ \midrule
\label{tab:multiclassvuln}
\end{tabular}
\end{table*}



\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\begin{algorithm}[H]
\caption{Graph Creation Algorithm}\label{alg:seqedge}
\begin{algorithmic}[1]

\Require \textit{code, edge\_length}: 

\Ensure Adjacency Matrix

\Procedure{\textit{SEQUENTIAL\_TOKEN\_EDGE}}{$tokens$}%\Comment{The g.c.d. of a and b}

%\State $params \gets getCmdLineParams(tokens)$



\For{$token$ in $tokens$}
    \State $nearbyTokens \gets getNearbyTokens(length)$
    \For{$next\_token$ in $nearbyTokens$}
        \If{$adj\_matr[token][next\_token]$ = $0$}
            \State $adj\_matr[token][next\_token] = 1$
        \EndIf
    \EndFor
    
    %\Comment{Logic For CWE Edges}
\EndFor


\EndProcedure

\end{algorithmic}
\end{algorithm}



\begin{table*}[t]
\centering
\caption{LSTD Edge Categories mapped with a set of CWE numbers. Each LSTD edge is responsible for the corresponding numbers. We also provide a short description for each edge category.}
\label{tab:graph}
\begin{tabular}{p{0.17\textwidth}
                p{0.19\textwidth}
                p{0.45\textwidth}
                 }
\toprule
\multicolumn{1}{l}{\textbf{CWE Number}} & \textbf{LSTD Edge Category} & \textbf{Short Description} \\
\midrule

%DATA\_FLOW  &   CWE-787,    &   Desc.   \\
% ASSIGNEMNT_EDGE
% OUT_OF_SCOPE
% NEXT_TOKEN
% CHECK_VALUE
% HARD_CODED_ASSIGNMENT/FORCED_ASSIGNMENT


119, 704, 369, 170, 676 & OPERATION\_CONSTRAINT     & Captures mathematical operations during assignment. \\

20, 190, 400, 665, 476  & CHECK\_VALUE     & Check value before assignment operations \\

74, 506 & CMD\_INJECTION     & Check before executing a command line argument \\

404, 666 & OUT\_OF\_SCOPE     & Usage of variable after free'd. \\

362, 662, 573 & RACE\_CONDITION     & An exclusive variable used out of synchronization  \\


\bottomrule
\end{tabular}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\color{red}
Appendix??? (Find Good Citations)
\paragraph{\textbf{Long-Range Dependencies}} We proposed the term long-range dependency to show the token distance between the declaration of a variable \textit{hostname} (Figure \ref{fig:code}, line 3) and its use (Figure \ref{fig:code}, line 8) of the same variable. Token distance implies the number of tokens between the usage of two variables/tokens. For example, in  figure \ref{fig:code} the token distance of the same variable \textit{hostname} is 18. However, this distance could be in the range of thousands or more in large programs. 
\color{black}


\begin{figure}[t]
    %\begin{framed}
        \centering
        
        \includegraphics[width=\textwidth]{eurosp2023-template/images/vuln.pdf}
        
    %\end{framed}
    \caption{An example of a vulnerability explanation provided to developers as part of an automated code review process to help developers effectively resolve static software security issues.
    }
    \label{fig:code}
\end{figure}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[ht]
\caption{A metadata of our curated VulF dataset with their corresponding CWE number, Poacher flow edges Edge Category and Description. The descriptions were provided by CWE \cite{cwe} }
\begin{tabular}{p{0.08\textwidth}
                p{0.08\textwidth}
                p{0.10\textwidth}
                p{0.55\textwidth}
                 }

\toprule
\textbf{CWE Label} & \textbf{Number of Functions} & \multicolumn{1}{l}{\textbf{Poacher Edge Category}}       & \textbf{Function Vulnerability Description}                                                                                                                                                                                                                                                                                          \\ \hline
Benign      & \multicolumn{1}{l|}{138522}  & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{l}{N/A}                                                                                                                                                                                                                                                                                      \\ \hline
CWE-119            & \multicolumn{1}{l|}{18618}   & \multicolumn{1}{c|}{\multirow{10}{*}{API\_ASSIGNMENT}} & {The software performs operations on a memory buffer, but it can read from or write to a memory location that is outside of the intended boundary of the buffer.}                                                                                                                          \\ \cline{1-2} \cline{4-4} 
CWE-704            & \multicolumn{1}{l|}{5251}    & \multicolumn{1}{c|}{}                                 & {The software does not correctly convert an object, resource, or structure from one type to a different type.}                                                                                                                                                                             \\ \cline{1-2} \cline{4-4} 
CWE-369            & \multicolumn{1}{l|}{289}     & \multicolumn{1}{c|}{}                                 & {The product divides a value by zero.}                                                                                                                                                                                                                                                     \\ \cline{1-2} \cline{4-4} 
CWE-170            & \multicolumn{1}{l|}{45}      & \multicolumn{1}{c|}{}                                 & {The software does not terminate or incorrectly terminates a string or array with a null character or equivalent terminator.}                                                                                                                                                              \\ \cline{1-2} \cline{4-4} 
CWE-676            & \multicolumn{1}{l|}{61}      & \multicolumn{1}{c|}{}                                 & {The program invokes a potentially dangerous function that could introduce a vulnerability if it is used incorrectly, but the function can also be used safely.}                                                                                                                           \\ \cline{1-2} \cline{4-4} 
CWE-20             & \multicolumn{1}{l|}{2703}    & \multicolumn{1}{c|}{}    & The product receives input or data, but it does not validate or incorrectly validates that the input has the properties that are required to process the data safely and correctly.                                                                                                                           \\ \cline{1-2} \cline{4-4} 
CWE-190            & \multicolumn{1}{l|}{326}     & \multicolumn{1}{c|}{}                                 & The software performs a calculation that can produce an integer overflow or wraparound, when the logic assumes that the resulting value will always be larger than the original value. This can introduce other weaknesses when the calculation is used for resource management or execution control.         \\ \cline{1-2} \cline{4-4} 
CWE-400            & \multicolumn{1}{l|}{3324}    & \multicolumn{1}{c|}{}                                 & The software does not properly control the allocation and maintenance of a limited resource, thereby enabling an actor to influence the amount of resources consumed, eventually leading to the exhaustion of available resources.                                                                            \\ \cline{1-2} \cline{4-4} 
CWE-665            & \multicolumn{1}{l|}{2022}    & \multicolumn{1}{c|}{}                                 & The software does not initialize or incorrectly initializes a resource, which might leave the resource in an unexpected state when it is accessed or used.                                                                                                                                                    \\ \cline{1-2} \cline{4-4} 
CWE-476            & \multicolumn{1}{l|}{1701}    & \multicolumn{1}{c|}{}                                 & A NULL pointer dereference occurs when the application dereferences a pointer that it expects to be valid, but is NULL, typically causing a crash or exit.                                                                                                                                                    \\ \hline
CWE-404            & \multicolumn{1}{l|}{2058}    & \multicolumn{1}{c|}{\multirow{2}{*}{OUT\_OF\_SCOPE}}  & The program does not release or incorrectly release a resource before it is made available for re-use.                                                                                                                                                                                                        \\ \cline{1-2} \cline{4-4} 
CWE-666            & \multicolumn{1}{l|}{580}     & \multicolumn{1}{c|}{}                                 & The software performs an operation on a resource at the wrong phase of the resource's lifecycle, which can lead to unexpected behaviors.                                                                                                                                                                      \\ \hline
CWE-74             & \multicolumn{1}{l|}{4021}    & \multicolumn{1}{c|}{\multirow{2}{*}{CMD\_INJECTION}}  & The software constructs all or part of a command, data structure, or record using externally-influenced input from an upstream component, but it does not neutralize or incorrectly neutralizes special elements that could modify how it is parsed or interpreted when it is sent to a downstream component. \\ \cline{1-2} \cline{4-4} 
CWE-506            & \multicolumn{1}{l|}{421}     & \multicolumn{1}{c|}{}                                 & The application contains code that appears to be malicious in nature.                                                                                                                                                                                                                                         \\ \hline
CWE-362            & \multicolumn{1}{l|}{211}     & \multicolumn{1}{c|}{\multirow{3}{*}{RACE\_CONDITION}} & The program contains a code sequence that can run concurrently with other code, and the code sequence requires temporary, exclusive access to a shared resource, but a timing window exists in which the shared resource can be modified by another code sequence that is operating concurrently.             \\ \cline{1-2} \cline{4-4} 
CWE-662            & \multicolumn{1}{l|}{221}     & \multicolumn{1}{c|}{}                                 & The software utilizes multiple threads or processes to allow temporary access to a shared resource that can only be exclusive to one process at a time, but it does not properly synchronize these actions, which might cause simultaneous accesses of this resource by multiple threads or processes.        \\ \cline{1-2} \cline{4-4} 
CWE-573            & \multicolumn{1}{l|}{331}     & \multicolumn{1}{c|}{}                                 & The software does not follow or incorrectly follows the specifications as required by the implementation language, environment, framework, protocol, or platform.                                                                                                                                             \\ \hline
                   & \multicolumn{1}{l|}{Total = 158001} & \multicolumn{1}{l|}{}                                 & \multicolumn{1}{l}{}                                                                                                                                                                                                                                                                                         \\ \hline
\label{tab:multiclassvuln}
\end{tabular}
\end{table*}



%%%%%%%%%%%

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[ht]
%\begin{tabular}{lcl|l}
\caption{Metadata of our curated VulF dataset with their corresponding CWE number, Poacher flow edge category and description. The descriptions were provided by CWE \cite{cwe}.}
\begin{tabular}{p{0.08\textwidth}
                p{0.08\textwidth}
                p{0.10\textwidth}
                p{0.55\textwidth}
                 }
\hline
\textbf{Number of Functions}        & \multicolumn{1}{l}{\textbf{LSTD Edge Category}}        & \textbf{CWE Label} & \textbf{Description}                                                                                                                                                                                                                                                                                          \\ \hline
\multicolumn{1}{l|}{138522}         & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{Non-Vulnerable}     & \multicolumn{1}{l}{N/A}                                                                                                                                                                                                                                                                                      \\ \hline
\multicolumn{1}{l|}{18618}          & \multicolumn{1}{c|}{\multirow{10}{*}{OPERATION\_EDGE}} & \multicolumn{1}{c|}{CWE-119}            & {The software performs operations on a memory buffer, but it can read from or write to a memory location that is outside of the intended boundary of the buffer.}                                                                                                                          \\ \cline{1-1} \cline{3-4} 
\multicolumn{1}{l|}{5251}           & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{CWE-704}            & {The software does not correctly convert an object, resource, or structure from one type to a different type.}                                                                                                                                                                             \\ \cline{1-1} \cline{3-4} 
\multicolumn{1}{l|}{289}            & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{CWE-369}            & {The product divides a value by zero.}                                                                                                                                                                                                                                                     \\ \cline{1-1} \cline{3-4} 
\multicolumn{1}{l|}{45}             & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{CWE-170}            & {The software does not terminate or incorrectly terminates a string or array with a null character or equivalent terminator.}                                                                                                                                                              \\ \cline{1-1} \cline{3-4} 
\multicolumn{1}{l|}{61}             & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{CWE-676}            & {The program invokes a potentially dangerous function that could introduce a vulnerability if it is used incorrectly, but the function can also be used safely.}                                                                                                                           \\ \cline{1-1} \cline{3-4} 
\multicolumn{1}{l|}{2703}           & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{CWE-20}             & The product receives input or data, but it does not validate or incorrectly validates that the input has the properties that are required to process the data safely and correctly.                                                                                                                           \\ \cline{1-1} \cline{3-4} 
\multicolumn{1}{l|}{326}            & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{CWE-190}            & The software performs a calculation that can produce an integer overflow or wraparound, when the logic assumes that the resulting value will always be larger than the original value. This can introduce other weaknesses when the calculation is used for resource management or execution control.         \\ \cline{1-1} \cline{3-4} 
\multicolumn{1}{l|}{3324}           & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{CWE-400}            & The software does not properly control the allocation and maintenance of a limited resource, thereby enabling an actor to influence the amount of resources consumed, eventually leading to the exhaustion of available resources.                                                                            \\ \cline{1-1} \cline{3-4} 
\multicolumn{1}{l|}{2022}           & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{CWE-665}            & The software does not initialize or incorrectly initializes a resource, which might leave the resource in an unexpected state when it is accessed or used.                                                                                                                                                    \\ \cline{1-1} \cline{3-4} 
\multicolumn{1}{l|}{1701}           & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{CWE-476}            & A NULL pointer dereference occurs when the application dereferences a pointer that it expects to be valid, but is NULL, typically causing a crash or exit.                                                                                                                                                    \\ \hline
\multicolumn{1}{l|}{2058}           & \multicolumn{1}{c|}{\multirow{2}{*}{OUT\_OF\_SCOPE}}   & \multicolumn{1}{c|}{CWE-404}            & The program does not release or incorrectly release a resource before it is made available for re-use.                                                                                                                                                                                                        \\ \cline{1-1} \cline{3-4} 
\multicolumn{1}{l|}{580}            & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{CWE-666}            & The software performs an operation on a resource at the wrong phase of the resource's lifecycle, which can lead to unexpected behaviors.                                                                                                                                                                      \\ \hline
\multicolumn{1}{l|}{4021}           & \multicolumn{1}{c|}{\multirow{2}{*}{CMD\_INJECTION}}   & \multicolumn{1}{c|}{CWE-74}             & The software constructs all or part of a command, data structure, or record using externally-influenced input from an upstream component, but it does not neutralize or incorrectly neutralizes special elements that could modify how it is parsed or interpreted when it is sent to a downstream component. \\ \cline{1-1} \cline{3-4} 
\multicolumn{1}{l|}{421}            & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{CWE-506}            & The application contains code that appears to be malicious in nature.                                                                                                                                                                                                                                         \\ \hline
\multicolumn{1}{l|}{211}            & \multicolumn{1}{c|}{\multirow{3}{*}{RACE\_CONDITION}}  & \multicolumn{1}{c|}{CWE-362}            & The program contains a code sequence that can run concurrently with other code, and the code sequence requires temporary, exclusive access to a shared resource, but a timing window exists in which the shared resource can be modified by another code sequence that is operating concurrently.             \\ \cline{1-1} \cline{3-4} 
\multicolumn{1}{l|}{221}            & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{CWE-662}            & The software utilizes multiple threads or processes to allow temporary access to a shared resource that can only be exclusive to one process at a time, but it does not properly synchronize these actions, which might cause simultaneous accesses of this resource by multiple threads or processes.        \\ \cline{1-1} \cline{3-4} 
\multicolumn{1}{l|}{331}            & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{CWE-573}            & The software does not follow or incorrectly follows the specifications as required by the implementation language, environment, framework, protocol, or platform.                                                                                                                                             \\ \hline
\multicolumn{1}{l|}{Total = 158001} & \multicolumn{1}{l|}{}                                  &                    & \multicolumn{1}{l}{}                                                                                                                                                                                                                                                                                         \\ \hline
\label{tab:multiclassvuln}

\end{tabular}
\end{table*}



%%%%%%%%%%%%%%%%%%%%%%


\begin{table*}[ht]
\caption{Metadata of our curated VulF dataset with their corresponding CWE number, Poacher Flow edge category and description. The descriptions were provided by CWE \cite{cwe}.}
\begin{tabular}{p{0.12\textwidth}
                p{0.70\textwidth}
                p{0.12\textwidth}
                 }
\hline
\textbf{Number of Functions} & \textbf{CWE Label} & \textbf{Description}                                                                                                                                                                                                                                                                                          \\ \hline
138522                       & Non-Vulnerable     & N/A                                                                                                                                                                                                                                                                                                          \\ \hline
18618                        & CWE-119            & The software performs operations on a memory buffer, but it can read from or write to a memory location that is outside of the intended boundary of the buffer.                                                                                                                                               \\ \hline
5251                         & CWE-704            & The software does not correctly convert an object, resource, or structure from one type to a different type.                                                                                                                                                                                                  \\ \hline

4021                         & CWE-74             & The software constructs all or part of a command, data structure, or record using externally-influenced input from an upstream component, but it does not neutralize or incorrectly neutralizes special elements that could modify how it is parsed or interpreted when it is sent to a downstream component. \\ \hline


1701                         & CWE-476            & A NULL pointer dereference occurs when the application dereferences a pointer that it expects to be valid, but is NULL, typically causing a crash or exit.                                                                                                                                                    \\ \hline


580                          & CWE-666            & The software performs an operation on a resource at the wrong phase of the resource's lifecycle, which can lead to unexpected behaviors.                                                                                                                                                                      \\ \hline

421                          & CWE-506            & The application contains code that appears to be malicious in nature.                                                                                                                                                                                                                                         \\ \hline

331                          & CWE-573            & The software does not follow or incorrectly follows the specifications as required by the implementation language, environment, framework, protocol, or platform.                                                                                                                                             \\ \hline

326                          & CWE-190            & The software performs a calculation that can produce an integer overflow or wraparound, when the logic assumes that the resulting value will always be larger than the original value. This can introduce other weaknesses when the calculation is used for resource management or execution control.         \\ \hline


289                          & CWE-369            & The product divides a value by zero.                                                                                                                                                                                                                                                                          \\ \hline

221                          & CWE-662            & The software utilizes multiple threads or processes to allow temporary access to a shared resource that can only be exclusive to one process at a time, but it does not properly synchronize these actions, which might cause simultaneous accesses of this resource by multiple threads or processes.        \\ \hline

211                          & CWE-362            & The program contains a code sequence that can run concurrently with other code, and the code sequence requires temporary, exclusive access to a shared resource, but a timing window exists in which the shared resource can be modified by another code sequence that is operating concurrently.             \\ \hline


61                           & CWE-676            & The program invokes a potentially dangerous function that could introduce a vulnerability if it is used incorrectly, but the function can also be used safely.                                                                                                                                                \\ \hline
Total = 158001               &                    &                                                                                                                                                                                                                                                                                                               \\ \hline
\label{tab:multiclassvuln}

\end{tabular}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{table}[t]
\centering
\caption{CWE prediction based on wild dataset. We mapped vulnerable data to their respective CWE numbers. This table also depicts how many CWEs our model can accurately predict.}
\label{tab:cwe}
\begin{tabular}{p{0.25\textwidth}
                 p{0.05\textwidth}
                 p{0.07  \textwidth}
                 }
\toprule
\multicolumn{1}{l}{\textbf{CWE Number}} & \textbf{Total} & \textbf{Correct Prediction} \\
\midrule
CWE-787: Out-of-bounds Write & 10 & 10 \\

CWE-20: Improper Input Validation  & 2 & 2 \\

CWE-125: Out-of-bounds Read & 1 & 1 \\

CWE-78: Improper Neutralization of Special Elements used in an OS Command  & 14 & 14 \\

CWE-416: Use After Free	 & 4 & 4 \\

CWE-476: NULL Pointer Dereference & 3 & \textbf{1}  \\

CWE-190: Integer Overflow or Wraparound & 9 & 9\\

CWE-798:Use of Hard-coded Credentials & 2 & 2 \\

CWE-77:Improper Neutralization of Special Elements used in a Command  & 2 & 2 \\



CWE-362: Concurrent Execution using Shared Resource with Improper Synchronization & 2 & 2 \\

CWE-400: Uncontrolled Resource Consumption & 5 & 5 \\

\midrule
 & 44 & 42  \\

\bottomrule


\end{tabular}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[t]
\label{novelpf}
\begin{tabular}{@{}ccccccc@{}}
\toprule
\multicolumn{1}{l}{\textbf{Input Method}} & \multicolumn{1}{l}{\textbf{API Calls}} & \multicolumn{1}{l}{\textbf{Assignment Operations}} & \multicolumn{1}{l}{\textbf{Execute Before Check}} & \multicolumn{1}{l}{\textbf{Code Injection}} & \multicolumn{1}{l}{\textbf{Free Variable}} & \multicolumn{1}{l}{\textbf{Incorrect Sync.}} \\ \midrule
PF                                        & Y                                      & Y                                                  & Y                                                 & Y                                           & Y                                          & Y                                            \\
AST                                       & N                                      & Y                                                  & N                                                 & N                                           & N                                          & N                                            \\
CPG (JOERN)                               & N                                      & Y                                                  & N                                                 & N                                           & N                                          & N                                            \\ \bottomrule
\end{tabular}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%   REVEAL %%%%%%%%

\multirow{6}{*}{ReVEAL}                          & \textbf{SVG}&\textbf{47.91}&\textbf{57.52}&\textbf{50.20}&\textbf{90.62}\\
& SVG w/o PF&45.54&55.01&48.34&89.47\\
& SVG+PF w/o DP&44.20&55.34&49.55&89.10\\
& SVG+PF w/o AC&46.12&56.89&47.85&89.10\\
& SVG+PF w/o RM&46.23&56.75&49.10&89.35\\ \hline



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[b]
    %\begin{framed}
        \centering
        
        \includegraphics[width=0.5\textwidth]{eurosp2023-template/images/acc_cwe.pdf}
        
    %\end{framed}
    \caption{The accuracy of our proposed Multitask RoBERTa-GCN vulnerability detection on our VulF dataset.}
    \label{fig:acc_per_cwe}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\section{Graph Creation Algorithms}
Here we explain how we generate our Data Control and Sequential Flow graph in addition to our Poacher Flow edges from Algorithm \ref{alg:algorithm_1}.

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\begin{algorithm}[H]
\caption{SVG Creation Algorithm}\label{alg:graph}
\begin{algorithmic}[1]

\Require \textit{code, edge\_length}: 

\Ensure Adjacency Matrix

\Procedure{\textit{SVG\_Generation}}{$code$}%\Comment{The g.c.d. of a and b}

\State $tokens \gets RoBERTaTokenizer(code)$

\State $cond\_statement$ = $for/if/while/else/else if$
%\State $CWE\_EDGE\_LIST \gets [Egde Types from Table \ref{tab:graph}]$
%\State $node \gets root$

\While{$token$ in $tokens$}%\Comment{We have the answer if r is 0}
    \State $type = checkTokernType(token)$
    \If{$type$ is $"variable"$}
        \State $var\_list.append(token)$
        \If{$token$ exists in $var\_list$}
            \State $prev\_token  \gets getPrevTok(token)$
            \State $adj\_matr[token][prev\_token]  \gets 1$
        \EndIf
        
    \EndIf
    
    \If{$token$ in $assignment_operators$}
        \State $left \gets getPrevToken(token)$
        \State $right \gets getNextToken(token)$
        
        \State $adj_matrix[left][right] \gets 1$
        
    \EndIf
    
    \Comment{Control Flow Edge Generate}
    \State $next \gets getNextToken(token)$
    \State $adj\_matr[token][next\_token]  \gets 1$
    \If{$type$ is in $"cond\_statements"$}
        
        \State $next\_token  \gets getNextBlockToken(token)$
        
        \State $adj\_matr[token][next\_token]  \gets 1$
           
            
        
        
    \EndIf 
\EndWhile\label{euclidendwhile1}

\State $OPERATION\_EDGE(tokens)$
\State $CHECK\_VALUE(tokens)$
\State $SCOPE\_RACE(tokens)$
\State $CMD\_INJECTION(tokens)$
\State $SEQUENTIAL\_TOKEN\_EDGE(tokens)$
 




\EndProcedure
\end{algorithmic}
\end{algorithm}




%\textbf{Sequential Token Edges:} We generate these edges at the end of our SVG generation procedures. These edges shows the remaining connections/edges that exists. To, generate this edge we create a token radius, and and create edges from the node to all the nodes within the token radius. Since these edges creates connection between the brackets and semicolons ("{", "}",";"), this helps the classifier to have a better syntactic understanding of the program.





% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[b]
\centering
\begin{tabular}{p{0.45\textwidth}
                 p{0.03\textwidth}
                 p{0.03\textwidth}
                 p{0.03\textwidth}
                 p{0.1\textwidth}
                 p{0.12\textwidth}}
\toprule
CWE                                                           & DP & AC & RM & Vulnerable & Non-Vulnerable \\ \midrule
CWE-601: URL Redirection to Untrusted Site ('Open Redirect')  & 10 & 8  & 10 & 5          & 5              \\
CWE-863: Incorrect Authorization                              & 10 & 7  & 9  & 5          & 4              \\
CWE-602: Client-Side Enforcement of Server-Side Security      & 11 & 3  & 6  & 5          & 5              \\
CWE-441: Unintended Proxy or Intermediary ('Confused Deputy') & 12 & 7  & 14 & 5          & 5              \\
CWE-799: Improper Control of Interaction Frequency            & 4  & 5  & 6  & 3          & 3              \\
CWE-352: Cross-Site Request Forgery (CSRF)                    & 1  & 8  & 0  & 3          & 3              \\
CWE-131: Incorrect Calculation of Buffer Size                 & 9  & 0  & 2  & 3          & 3              \\
CWE-134: Uncontrolled Format String                           & 10 & 0  & 4  & 5          & 5              \\
CWE-197: Numeric Truncation Error                             & 10 & 0  & 0  & 4          & 4              \\
CWE-252: Unchecked Return Value                               & 8  & 0  & 0  & 6          & 2              \\
CWE-481: Assigning Instead of Comparing                       & 1  & 8  & 4  & 3          & 3              \\
CWE-617: Reachable Assertion                                  & 6  & 0  & 3  & 3          & 3              \\
CWE-788: Access of Memory Location After End of Buffer        & 6  & 8  & 4  & 3          & 3              \\
CWE-338: Use of Cryptographically Weak PRNG                   & 9  & 0  & 0  & 4          & 5              \\
CWE-415: Double Free                                          & 0  & 0  & 8  & 4          & 4              \\
CWE-457: Use of Uninitialized Variable                        & 12 & 0  & 0  & 4          & 4              \\
CWE-571: Expression is Always False/True                      & 5  & 0  & 0  & 2          & 3              \\
CWE-690: NULL Pointer Dereference in a Condition              & 6  & 6  & 0  & 3          & 3              \\ \bottomrule
\end{tabular}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[b]
\centering
\caption{Accuracy, Precision, Recall and F1 scores of our proposed Multitask RoBERTa-GCN with various input types on our VulF dataset.}
    \label{tab:acc_per_cwe}
\begin{tabular}{@{}llllll@{}}
\toprule
Dataset               & Model             & Accuracy       & Prec.          & Recall         & F1             \\ \midrule
\multirow{4}{*}{VulF} & RoBERTa-PFGCN     & \textbf{96.24} & \textbf{96.18} & \textbf{95.15} & \textbf{95.85} \\
                      & Devign            & 84.55          & 83.94          & 83.15          & 84.30          \\
                      & VELVET            & 84.45          & 85.12          & 85.20          & 84.46          \\
                      & $\mu$VulDeePecker & 78.35          & 78.94          & 78.30          & 77.10          \\ \bottomrule
\end{tabular}
\end{table}




%%%%%%%%%%% Updated Metadata Table %%%%%%%%%%%%%%%%
\begin{table*}[ht]
\caption{Summary of our VulF dataset with total number of functions for each CWE labels with \color{red} short \color{black} description. The \color{red} short \color{black} descriptions were provided by CWE \cite{cwe}.}
\begin{tabular}{p{0.12\textwidth}
                p{0.70\textwidth}
                p{0.12\textwidth}
                 }
\hline
\textbf{Functions} & \textbf{Short Description} & \textbf{CWE Label}                                                                                                                                                                                                                                                                                          \\ \hline
138522                       &  N/A    & Non-Vulnerable                                                                                                                                                                                                                                                                                                          \\ \hline
18618                        & The software performs operations on a memory buffer, but it can read from or write to a memory location that is outside of the intended boundary of the buffer.            &  CWE-119                                                                                                                                              \\ \hline
5251                         & The software does not correctly convert an object, resource, or structure from one type to a different type.            &    CWE-704                                                                                                                                                                                               \\ \hline

4021                         & The software constructs all or part of a command, data structure, or record using externally-influenced input from an upstream component, but it does not neutralize or incorrectly neutralizes special elements that could modify how it is parsed or interpreted when it is sent to a downstream component.             &  CWE-74 \\ \hline


1701                         & A NULL pointer dereference occurs when the application dereferences a pointer that it expects to be valid, but is NULL, typically causing a crash or exit.            &    CWE-476                                                                                                                                                 \\ \hline



421                          & The application contains code that appears to be malicious in nature.            &       CWE-506                                                                                                                                                                                                                                   \\ \hline

331                          & The software does not follow or incorrectly follows the specifications as required by the implementation language, environment, framework, protocol, or platform.            &     CWE-573                                                                                                                                         \\ \hline

326                          & The software performs a calculation that can produce an integer overflow or wraparound, when the logic assumes that the resulting value will always be larger than the original value. This can introduce other weaknesses when the calculation is used for resource management or execution control.             &    CWE-190     \\ \hline


289                          & The product divides a value by zero.            &     CWE-369                                                                                                                                                                                                                                                                      \\ \hline

221                          & The software utilizes multiple threads or processes to allow temporary access to a shared resource that can only be exclusive to one process at a time, but it does not properly synchronize these actions, which might cause simultaneous accesses of this resource by multiple threads or processes.            &      CWE-662   \\ \hline

211                          & The program contains a code sequence that can run concurrently with other code, and the code sequence requires temporary, exclusive access to a shared resource, but a timing window exists in which the shared resource can be modified by another code sequence that is operating concurrently.            &    CWE-362           \\ \hline


61                           & The program invokes a potentially dangerous function that could introduce a vulnerability if it is used incorrectly, but the function can also be used safely.            &          CWE-676                                                                                                                                       \\ \hline
Total = 144678               &                    &                                                                                                                                                                                                                                                                                                               \\ \hline
\label{tab:multiclassvuln}

\end{tabular}
\end{table*}




%%%%% TAble 8 Ablation


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[ht]
\centering
\caption{\color{red} In-depth ablation study for each component of our proposed PF Edges\color{black}}
\label{tab:ablation_2}
\begin{tabular}{p{0.08\textwidth}
                 p{0.14\textwidth}
                 p{0.03\textwidth}
                 p{0.02\textwidth}
                 p{0.02\textwidth}
                 p{0.02\textwidth}}
%\begin{tabular}{clllll}
\toprule
\textbf{Dataset}                                 & \multicolumn{1}{l}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Acc.}} & \multicolumn{1}{c}{\textbf{Prec.}} & \multicolumn{1}{c}{\textbf{Recall}} & \multicolumn{1}{c}{\textbf{F1}} \\ \midrule




%{500-VulF + 144-CWE}
\multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}VulF\end{tabular}} & GCN                           & 87.50                                      & 87.36                                       &                  87.94                  &       87.23       \\
                                                 

& GCN w/ AC    & 91.23                                      & 91.75                                       &                  91.56                   &       91.23       \\              



& GCN w/ DP     & 90.40                                      & 89.65                                       &                  90.95                   &       90.50       \\                      
                                                 

                                            
& GCN w/ RM    & 89.54                                      & 90.28                                       &                  90.61                   &       90.83       \\                        



&  \textbf{RoBERTa-PFGCN}  & \textbf{96.24}                                    &               \textbf{96.18}&     \textbf{95.15}&                       \textbf{95.85} \\
\hline


%%%%



%%%%
\multirow{6}{*}{MVD}  & GCN&96.59&96.12&96.10&96.58\\

& GCN w/ AC&97.30&96.29&96.87&97.46\\
& GCN w/ DP&96.84&96.54&96.71&97.71\\


& GCN w/ RM&96.95&96.92&96.50&96.94\\ 

& \textbf{RoBERTa-PFGCN}&\textbf{98.01}&\textbf{98.28}&\textbf{98.23}&\textbf{98.23}\\
\hline
%\multicolumn{1}{l}{\multirow{6}{*}{FFMpeg}} 

%%%%%%%%%%%%%%

\multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}500-MVD +\\144-CWE\end{tabular}} & GCN                           & 86.10                                      & 85.75                                       &                  85.24                  &       86.50       \\
& GCN w/ AC    & 92.16                                      & 91.90                                       &                  91.10                   &       91.70       \\              
& GCN w/ DP     & 91.70                                      & 90.15                                       &                  91.57                   &       90.30       \\                    
& GCN w/ RM    & 91.46                                      & 92.40                                       &                  91.43                   &       91.33       \\                    
& \textbf{RoBERTa-PFGCN}&\textbf{97.80}&\textbf{98.75}&\textbf{98.10}&\textbf{98.28}\\
\hline

%%%%%%%%%%%%%%

\multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}FFMpeg\\ +Qemu\end{tabular}}  & GCN                              &60.48&61.10&60.04&60.34\\

%\multicolumn{1}{l}{}                             
%\multicolumn{1}{l}{}                             

\multicolumn{1}{l}{}                             & GCN w/ AC                           & 60.81                                      &     61.34                                   &        62.58                             &                  60.97               \\

\multicolumn{1}{l}{}                             & GCN w/ DP                           & 61.59                                      &     61.80                                   &        62.03                             &                  60.57               \\

\multicolumn{1}{l}{}                             & GCN w/ RM                           & 62.10                                      &     62.05                                   &        62.90                             &                  61.60               \\

& \textbf{RoBERTa-PFGCN}                                     &\textbf{62.99}&\textbf{63.08}&\textbf{62.97}&\textbf{63.29}\\
\hline



%%%%%%%%%%%%%%

\multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}500-FFMpeg +\\Qemu\\ +144-CWE\end{tabular}} & GCN                           & 56.34                                      & 57.47                                       &                  57.28                  &       56.57       \\
& GCN w/ AC    & 60.94                                      & 60.12                                       &                  60.35                   &       60.48       \\              
& GCN w/ DP     & 61.50                                      & 60.51                                       &                  61.23                   &       60.80       \\                    
& GCN w/ RM    & 61.90                                      & 61.08                                       &                  61.40                   &       61.74       \\                    
& \textbf{RoBERTa-PFGCN}&\textbf{65.10}&\textbf{64.29}&\textbf{65.85}&\textbf{64.10}\\
\hline

%%%%%%%%%%%%%%



\multirow{6}{*}{D2A}
& GCN&56.10&59.86&60.21&59.71\\
                                                 

& GCN w/ AC                           & 59.92                                      & 60.10                                       &                  60.29                   &       60.50       \\

& GCN w/ DP                           & 59.12                                      & 60.89                                       &                  61.20                   &       60.74       \\
                                                 

                                            
& GCN w/ RM                           & 61.12                                      & 61.01                                       &                  61.70                   &       60.74       \\ 

& \textbf{RoBERTa-PFGCN}&\textbf{61.21}&\textbf{61.97}&\textbf{62.07}&\textbf{61.20}\\
\hline


%%%%%%%%%%%%%%

\multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}500-D2A\\ +144-CWE\end{tabular}} & GCN                           & 57.95                                      & 58.80                                       &                  57.69                  &       58.46       \\
& GCN w/ AC    & 61.29                                      & 62.50                                       &                  61.58                   &       62.20       \\              
& GCN w/ DP     & 61.65                                      & 60.10                                       &                  61.95                   &       60.28       \\                    
& GCN w/ RM    & 60.30                                      & 59.28                                       &                  59.10                   &       59.25       \\                    
& \textbf{RoBERTa-PFGCN}&\textbf{66.50}&\textbf{66.90}&\textbf{66.10}&\textbf{65.92}\\


%%%%%%%%%%%%%%



\bottomrule



\end{tabular}
\end{table}



\and
\IEEEauthorblockN{2\textsuperscript{nd} Gonzalo De La Torre Parra}
\IEEEauthorblockA{\textit{University of the Incarnate Word} \\
%City, Country \\
gdparra@uiwtx.edu}
\and
\IEEEauthorblockN{3\textsuperscript{rd} Dylan Manuel}
\IEEEauthorblockA{\textit{University of Texas at San Antonio} \\
%City, Country \\
dylan.manuel@my.utsa.edu}
\and
\IEEEauthorblockN{4\textsuperscript{th} Elias Bou-Harb}
\IEEEauthorblockA{\textit{University of Texas at San Antonio} \\
%City, Country \\
elias.bouharb@utsa.edu}
\and
\IEEEauthorblockN{5\textsuperscript{th} Peyman Najafirad}
\IEEEauthorblockA{\textit{University of Texas at San Antonio} \\
%City, Country \\
peyman.najafirad@utsa.edu}
%% IEEE format can accommodate up to six authors this way
}
